Electrostatic Bender Optics

The relativistically-correct Hamiltonian and transfer matrix of electrostatic benders is derived. This is the general case where the bender electrodes have curvature in the non-bend direction.

==> cover_page_macro.tex <==
%
% produces cover for design reports
%
% inputs are;
% 1 - File number (eg. TRI-DN-88-10)
% 2 - Author(s)
% 3 - Title
% 4 - Abstract
% 5 - Design note date
%
\def\make_cover_page#1#2#3#4#5\par
{
\begin{titlepage}
%\pagenumbering set to alpha else hyperref complains. Have to set
 %\pagenumbering{arabic} in the main document
\pagenumbering{alph}
\thispagestyle{empty}
\setlength{\topmargin}{-0.8in}
\setlength{\parskip}{4.0mm}
\setlength{\textwidth}{8.5in}
\setlength{\parindent}{0pt}
 
%Apparently, the preferred font on title page is sans serif
 \sf
 
% Upper part of the page
\begin{minipage}{0.3\textwidth}
\begin{flushleft} \large
\includegraphics[width=\textwidth]{cov_page_logo}
%note the lack of an extension to the logo file. This means it will
 %choose a ps version for dvips, and a pdf (or png) version for pdflatex.
\end{flushleft}
\end{minipage}
\begin{minipage}[b]{0.4\textwidth}
\begin{flushright} \large
\textbf{TRIUMF Beam Physics Note} \\
#1\\
\setbox3=\hbox{#5}
%If date is too short, or empty, today is used.
\ifdim\wd3<30pt
  \today
 \else
  #5
 \fi
\end{flushright}
\end{minipage}
 \vspace{0.5in}
 
% Title
\begin{center}
  { \huge \bfseries #3}\\[0.5cm]

{ \Large \emph{#2}\\[0.5cm]
\emph{TRIUMF}}
\end{center}
{\large {\bfseries Abstract:} #4}
 
\vfill
 \footnotesize
% Bottom of the page
 4004 Wesbrook Mall, Vancouver, B.C. Canada V6T 2A3 · Tel: 604 222-1047 · Fax: 604 222-1074 · www.triumf.ca
\end{titlepage}
%
% now set things up for the next page
%
\markright{#1}
\newpage
\vsize=8.5in
\hsize=5.5in
%
% macro closing bracket
%
}

